Analyzing Learned Representations of a Deep ASR Performance Prediction Model

This paper addresses a relatively new task: prediction of ASR performance on unseen broadcast programs. In a previous paper, we presented an ASR performance prediction system using CNNs that encode both text (ASR transcript) and speech, in order to predict word error rate. This work is dedicated to the analysis of speech signal embeddings and text embeddings learnt by the CNN while training our prediction model. We try to better understand which information is captured by the deep model and its relation with different conditioning factors. It is shown that hidden layers convey a clear signal about speech style, accent and broadcast type. We then try to leverage these 3 types of information at training time through multi-task learning. Our experiments show that this allows to train slightly more efficient ASR performance prediction systems that - in addition - simultaneously tag the analyzed utterances according to their speech style, accent and broadcast program origin.

==> emnlp2018 <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Saved with string encoding Unicode (UTF-8) 

@inproceedings{elloumi2018asr,
  title={ASR PERFORMANCE PREDICTION ON UNSEEN BROADCAST PROGRAMS USING CONVOLUTIONAL NEURAL NETWORKS},
  author={Elloumi, Zied and Besacier, Laurent and Galibert, Olivier and Kahn, Juliette and Lecouteux, Benjamin},
  booktitle={IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  
  year={2018}
}

@inproceedings{elloumi2018asr_anonymous,
  title={anonymous},
  author={Elloumi, Zied and Besacier, Laurent and Galibert, Olivier and Kahn, Juliette and Lecouteux, Benjamin},
  booktitle={IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  year={2018}
}
@article{vylomova2016word,
  title={Word representation models for morphologically rich languages in neural machine translation},
  author={Vylomova, Ekaterina and Cohn, Trevor and He, Xuanli and Haffari, Gholamreza},
  journal={arXiv preprint arXiv:1606.04217},
  year={2016}
}
@article{DBLP:journals/corr/WuK16,
  author    = {Zhizheng Wu and
               Simon King},
  title     = {Investigating gated recurrent neural networks for speech synthesis},
  journal   = {CoRR},
  volume    = {abs/1601.02539},
  year      = {2016},
  url       = {http://arxiv.org/abs/1601.02539},
  archivePrefix = {arXiv},
  eprint    = {1601.02539},
  timestamp = {Wed, 07 Jun 2017 14:41:44 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/WuK16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/Sennrich16,
  author    = {Rico Sennrich},
  title     = {How Grammatical is Character-level Neural Machine Translation? Assessing
               {MT} Quality with Contrastive Translation Pairs},
  journal   = {CoRR},
  volume    = {abs/1612.04629},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.04629},
  archivePrefix = {arXiv},
  eprint    = {1612.04629},
  timestamp = {Wed, 07 Jun 2017 14:43:09 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/Sennrich16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



 
@article{hinton2012deep,
  title={Deep neural networks for acoustic modeling in speech recognition: The shared views of four research groups},
  author={Hinton, Geoffrey and Deng, Li and Yu, Dong and Dahl, George E and Mohamed, Abdel-rahman and Jaitly, Navdeep and Senior, Andrew and Vanhoucke, Vincent and Nguyen, Patrick and Sainath, Tara N and others},
  journal={IEEE Signal Processing Magazine},
  volume={29},
  number={6},
  pages={82--97},
  year={2012},
  publisher={IEEE}
}
@inproceedings{lai2015recurrent,
  title={Recurrent Convolutional Neural Networks for Text Classification.},
  author={Lai, Siwei and Xu, Liheng and Liu, Kang and Zhao, Jun},
  booktitle={AAAI},
  volume={333},
  pages={2267--2273},
  year={2015}
}

@article{kim2014convolutional,
  title={Convolutional neural networks for sentence classification},
  author={Kim, Yoon},
  journal={arXiv preprint arXiv:1408.5882},
  year={2014}
}

@inproceedings{graves2013speech,
  title={Speech recognition with deep recurrent neural networks},
  author={Graves, Alex and Mohamed, Abdel-rahman and Hinton, Geoffrey},
  booktitle={Acoustics, speech and signal processing (icassp), 2013 ieee international conference on},
  pages={6645--6649},
  year={2013},
  organization={IEEE}
}

@article{klein2017opennmt,
  title={Opennmt: Open-source toolkit for neural machine translation},
  author={Klein, Guillaume and Kim, Yoon and Deng, Yuntian and Senellart, Jean and Rush, Alexander M},
  journal={arXiv preprint arXiv:1701.02810},
  year={2017}
}

@article{wu2016google,
  title={Google's neural machine translation system: Bridging the gap between human and machine translation},
  author={Wu, Yonghui and Schuster, Mike and Chen, Zhifeng and Le, Quoc V and Norouzi, Mohammad and Macherey, Wolfgang and Krikun, Maxim and Cao, Yuan and Gao, Qin and Macherey, Klaus and others},
  journal={arXiv preprint arXiv:1609.08144},
  year={2016}
}
@article{DBLP:journals/corr/LuongLSVK15,
  author    = {Minh{-}Thang Luong and
               Quoc V. Le and
               Ilya Sutskever and
               Oriol Vinyals and
               Lukasz Kaiser},
  title     = {Multi-task Sequence to Sequence Learning},
  journal   = {CoRR},
  volume    = {abs/1511.06114},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.06114},
  archivePrefix = {arXiv},
  eprint    = {1511.06114},
  timestamp = {Wed, 07 Jun 2017 14:41:33 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/LuongLSVK15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{dong2015multi,
  title={Multi-task learning for multiple language translation},
  author={Dong, Daxiang and Wu, Hua and He, Wei and Yu, Dianhai and Wang, Haifeng},
  booktitle={Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  volume={1},
  pages={1723--1732},
  year={2015}
}
@article{DBLP:journals/corr/abs-1708-00993,
  author    = {Jan Niehues and
               Eunah Cho},
  title     = {Exploiting Linguistic Resources for Neural Machine Translation Using
               Multi-task Learning},
  journal   = {CoRR},
  volume    = {abs/1708.00993},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.00993},
  archivePrefix = {arXiv},
  eprint    = {1708.00993},
  timestamp = {Tue, 05 Sep 2017 10:03:46 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1708-00993},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
 
@inproceedings{seltzer2013multi,
  title={Multi-task learning in deep neural networks for improved phoneme recognition},
  author={Seltzer, Michael L and Droppo, Jasha},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2013 IEEE International Conference on},
  pages={6965--6969},
  year={2013},
  organization={IEEE}
}

@misc{
hsieh2018multitask,
title={Multi-task Learning on {MNIST} Image Datasets},
author={Po-Chen Hsieh and Chia-Ping Chen},
year={2018},
url={https://openreview.net/forum?id=S1PWi_lC-},
}

@article{liu2015representation,
  title={Representation learning using multi-task deep neural networks for semantic classification and information retrieval},
  author={Liu, Xiaodong and Gao, Jianfeng and He, Xiaodong and Deng, Li and Duh, Kevin and Wang, Ye-Yi},
  year={2015}
}
@inproceedings{ghoshal2013multilingual,
  title={Multilingual training of deep neural networks},
  author={Ghoshal, Arnab and Swietojanski, Pawel and Renals, Steve},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2013 IEEE International Conference on},
  pages={7319--7323},
  year={2013},
  organization={IEEE}
}
 

@article{liu2017adversarial,
  title={Adversarial multi-task learning for text classification},
  author={Liu, Pengfei and Qiu, Xipeng and Huang, Xuanjing},
  journal={arXiv preprint arXiv:1704.05742},
  year={2017}
}
@article{liu2016recurrent,
  title={Recurrent neural network for text classification with multi-task learning},
  author={Liu, Pengfei and Qiu, Xipeng and Huang, Xuanjing},
  journal={arXiv preprint arXiv:1605.05101},
  year={2016}
}
@inproceedings{huang2013cross,
  title={Cross-language knowledge transfer using multilingual deep neural network with shared hidden layers},
  author={Huang, Jui-Ting and Li, Jinyu and Yu, Dong and Deng, Li and Gong, Yifan},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2013 IEEE International Conference on},
  pages={7304--7308},
  year={2013},
  organization={IEEE}
}
@inproceedings{chen2014joint,
  title={Joint acoustic modeling of triphones and trigraphemes by multi-task learning deep neural networks for low-resource speech recognition},
  author={Chen, Dongpeng and Mak, Brian and Leung, Cheung-Chi and Sivadas, Sunil},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2014 IEEE International Conference on},
  pages={5592--5596},
  year={2014},
  organization={IEEE}
}
@inproceedings{mohan2015multi,
  title={Multi-lingual speech recognition with low-rank multi-task deep neural networks},
  author={Mohan, Aanchan and Rose, Richard},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2015 IEEE International Conference on},
  pages={4994--4998},
  year={2015},
  organization={IEEE}
}

@inproceedings{collobert2008unified,
  title={A unified architecture for natural language processing: Deep neural networks with multitask learning},
  author={Collobert, Ronan and Weston, Jason},
  booktitle={Proceedings of the 25th international conference on Machine learning},
  pages={160--167},
  year={2008},
  organization={ACM}
}
@article{maaten2008visualizing,
  title={Visualizing data using t-SNE},
  author={Maaten, Laurens van der and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={Nov},
  pages={2579--2605},
  year={2008}
}
@article{luong2015multi,
  title={Multi-task sequence to sequence learning},
  author={Luong, Minh-Thang and Le, Quoc V and Sutskever, Ilya and Vinyals, Oriol and Kaiser, Lukasz},
  journal={arXiv preprint arXiv:1511.06114},
  year={2015}
}


@article{toshniwal2017multilingual,
  title={Multilingual Speech Recognition With A Single End-To-End Model},
  author={Toshniwal, Shubham and Sainath, Tara N and Weiss, Ron J and Li, Bo and Moreno, Pedro and Weinstein, Eugene and Rao, Kanishka},
  journal={arXiv preprint arXiv:1711.01694},
  year={2017}
}

@article{johnson2016google,
  title={Google's multilingual neural machine translation system: enabling zero-shot translation},
  author={Johnson, Melvin and Schuster, Mike and Le, Quoc V and Krikun, Maxim and Wu, Yonghui and Chen, Zhifeng and Thorat, Nikhil and Vi{\'e}gas, Fernanda and Wattenberg, Martin and Corrado, Greg and others},
  journal={arXiv preprint arXiv:1611.04558},
  year={2016}
}

@inproceedings{wang2017does,
  title={What Does the Speaker Embedding Encode?},
  author={Wang, Shuai and Qian, Yanmin and Yu, Kai},
  booktitle={Interspeech},
  volume={2017},
  pages={1497--1501},
  year={2017}
}

@article{DBLP:journals/corr/KingmaB14,
  author    = {Diederik P. Kingma and
               Jimmy Ba},
  title     = {Adam: {A} Method for Stochastic Optimization},
  journal   = {CoRR},
  volume    = {abs/1412.6980},
  year      = {2014},
  url       = {http://arxiv.org/abs/1412.6980},
  archivePrefix = {arXiv},
  eprint    = {1412.6980},
  timestamp = {Wed, 07 Jun 2017 14:40:52 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KingmaB14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
 
@inproceedings{shi2016does,
  title={Does string-based neural MT learn source syntax?},
  author={Shi, Xing and Padhi, Inkit and Knight, Kevin},
  booktitle={Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing},
  pages={1526--1534},
  year={2016}
}
@inproceedings{dalvi2017understanding,
  title={Understanding and Improving Morphological Learning in the Neural Machine Translation Decoder},
  author={Dalvi, Fahim and Durrani, Nadir and Sajjad, Hassan and Belinkov, Yonatan and Vogel, Stephan},
  booktitle={Proceedings of the Eighth International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  volume={1},
  pages={142--151},
  year={2017}
}
@article{belinkov2017neural,
  title={What do Neural Machine Translation Models Learn about Morphology?},
  author={Belinkov, Yonatan and Durrani, Nadir and Dalvi, Fahim and Sajjad, Hassan and Glass, James},
  journal={arXiv preprint arXiv:1704.03471},
  year={2017}
}
@article{yu2013feature,
  title={Feature learning in deep neural networks-studies on speech recognition tasks},
  author={Yu, Dong and Seltzer, Michael L and Li, Jinyu and Huang, Jui-Ting and Seide, Frank},
  journal={arXiv preprint arXiv:1301.3605},
  year={2013}
}

@inproceedings{mohamed2012understanding,
  title={Understanding how deep belief networks perform acoustic modelling},
  author={Mohamed, Abdel-rahman and Hinton, Geoffrey and Penn, Gerald},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2012 IEEE International Conference on},
  pages={4273--4276},
  year={2012},
  organization={IEEE}
}
@inproceedings{belinkov2017analyzing,
  title={Analyzing Hidden Representations in End-to-End Automatic Speech Recognition Systems},
  author={Belinkov, Yonatan and Glass, James},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2438--2448},
  year={2017}
}

  

@inproceedings{belinkov2017evaluating,
  title={Evaluating Layers of Representation in Neural Machine Translation on Part-of-Speech and Semantic Tagging Tasks},
  author={Belinkov, Yonatan and M{\`a}rquez, Llu{\'\i}s and Sajjad, Hassan and Durrani, Nadir and Dalvi, Fahim and Glass, James},
  booktitle={Proceedings of the Eighth International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  volume={1},
  pages={1--10},
  year={2017}
}



@article{collobert2011natural,
  title={Natural language processing (almost) from scratch},
  author={Collobert, Ronan and Weston, Jason and Bottou, L{\'e}on and Karlen, Michael and Kavukcuoglu, Koray and Kuksa, Pavel},
  journal={Journal of Machine Learning Research},
  volume={12},
  number={Aug},
  pages={2493--2537},
  year={2011}
}

@inproceedings{jin2016lid,
  title={LID-senone extraction via deep neural networks for end-to-end language identification},
  author={Jin, Ma and Song, Yan and Mcloughlin, Ian and Dai, Li-Rong and Ye, Zhong-Fu},
  booktitle={Proc. of Odyssey},
  year={2016}
}

@inproceedings{piczak2015environmental,
  title={Environmental sound classification with convolutional neural networks},
  author={Piczak, Karol J},
  booktitle={Machine Learning for Signal Processing (MLSP), 2015 IEEE 25th International Workshop on},
  pages={1--6},
  year={2015},
  organization={IEEE}
}

@inproceedings{sainath2015learning,
  title={Learning the speech front-end with raw waveform CLDNNs},
  author={Sainath, Tara N and Weiss, Ron J and Senior, Andrew and Wilson, Kevin W and Vinyals, Oriol},
  booktitle={Sixteenth Annual Conference of the International Speech Communication Association},
  year={2015}
}
@article{ge2017neural,
  title={Neural Network Based Speaker Classification and Verification Systems with Enhanced Features},
  author={Ge, Zhenhao and Iyer, Ananth N and Cheluvaraja, Srinath and Sundaram, Ram and Ganapathiraju, Aravind},
  journal={arXiv preprint arXiv:1702.02289},
  year={2017}
}

@inproceedings{palaz2015convolutional,
  title={Convolutional neural networks-based continuous speech recognition using raw speech signal},
  author={Palaz, Dimitri and Doss, Mathew Magimai- and Collobert, Ronan},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2015 IEEE International Conference on},
  pages={4295--4299},
  year={2015},
  organization={IEEE}
}


@article{adelta,
  author    = {Matthew D. Zeiler},
  title     = {{ADADELTA:} An Adaptive Learning Rate Method},
  journal   = {CoRR},
  volume    = {abs/1212.5701},
  year      = {2012},
  url       = {http://arxiv.org/abs/1212.5701},
  timestamp = {Wed, 07 Jun 2017 14:43:02 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1212-5701},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{CNNrawWav,
  title={Very deep convolutional neural networks for raw waveforms},
  author={Dai, Wei and Dai, Chia and Qu, Shuhui and Li, Juncheng and Das, Samarjit},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2017 IEEE International Conference on},
  pages={421--425},
  year={2017},
  organization={IEEE}
}



@inproceedings{jalalvand2015stacked,
  title={Stacked auto-encoder for ASR error detection and word error rate prediction.},
  author={Jalalvand, Shahab and Falavigna, Daniele},
  booktitle={INTERSPEECH},
  pages={2142--2146},
  year={2015}
}

@inproceedings{zhang06,
	Address = {Sydney},
	Author = {Ying Zhang and Almut Silja Hildebrand and Stephan Vogel},
	Booktitle = {Proceedings of the 2006 Conference on Empirical Methods in Natural Language Processing (EMNLP 2006)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {July},
	Pages = {216-223},
	Title = {Distributed Language Modeling for N-best List Re-ranking},
	Year = {2006}}

@conference{zens06,
	Address = {Stroudsburg, PA, USA},
	Author = {Richard Zens and Hermann Ney},
	Booktitle = {Workshop on Statistical Machine Translation - StatMT},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {N-gram posterior probabilities for statistical machine translation},
	Year = {2006}}

@article{Young1994,
	Author = {Young, Sheryl R.},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Proc. of International Conference on Acoustics, Speech and Signal Processing},
	Pages = {21-24},
	Title = {Recognition Confidence Measures: Detection of Misrecognitions and Out-Of-Vocabulary Words},
	Year = {1994}}

@inproceedings{Xiong2010,
	Address = {Uppsala, Sweden},
	Author = {Deyi Xiong and Min Zhang and Haizhou Li},
	Booktitle = {Proceedings of the 48th annual meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {July},
	Pages = {604-611},
	Title = {Error Detection for Statistical Machine Translation Using Linguistic Features},
	Year = {2010}}

@inproceedings{xiong10,
	Address = {Uppsala, Sweden},
	Author = {Deyi Xiong and Min Zhang and Haizhou Li},
	Booktitle = {Proceedings of the 48th Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {July},
	Owner = {lent},
	Pages = {604-611},
	Timestamp = {2015.05.12},
	Title = {Error Detection for Statistical Machine Translation Using Linguistic Features},
	Year = {2010}}

@techreport{WordNet,
	Author = {{Princeton University}},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Institution = {Princeton University},
	Title = {"About WordNet"},
	Url = {http://WordNet.princeton.edu},
	Year = {2012},
	Bdsk-Url-1 = {http://WordNet.princeton.edu}}

@inproceedings{Wisniewski2014,
	Address = {Baltimore, Maryland, USA},
	Author = {Wisniewski, Guillaume and P\'{e}cheux, Nicolas and Allauzen, Alexander and Yvon, Fran\c{c}ois},
	Booktitle = {Proceedings of the Ninth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Owner = {Christophe},
	Pages = {348--354},
	Publisher = {Association for Computational Linguistics},
	Timestamp = {2015.09.24},
	Title = {LIMSI Submission for WMT'14 QE Task},
	Year = {2014}}

@inproceedings{wilker12,
	Address = {Istanbul, Turkey},
	Author = {Wilker Aziz and Sheila C. M. de Sousa and Lucia Specia},
	Booktitle = {Proceedings of the Eight International Conference on Language Resources and Evaluation (LREC'12)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {May 23-25},
	Title = {PET: a Tool for Post-editing and Assessing Machine Translation},
	Year = {2012}}

@article{wessel2001,
	Author = {Frank Wessel and Ralf Schl{\"u}ter and Klaus Macherey and Hermann Ney},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {IEEE TRANSACTIONS ON SPEECH AND AUDIO PROCESSING},
	Owner = {lent},
	Timestamp = {2015.05.12},
	Title = {Confidence Measures for Large Vocabulary Continuous Speech Recognition},
	Year = {2001}}

@inproceedings{watanabe07,
	Address = {Prague, Czech Republic},
	Author = {Taro Watanabe and Jun Suzuki and Hajime Tsukada and Hideki Isozaki},
	Booktitle = {Proceedings of the 2007 Joint Conference on Empirical Methods in Natural Language Processing and Computational Natural Language Learning},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Pages = {64--773,},
	Title = {Online Large-Margin Training for Statistical Machine Translation},
	Year = {2007}}

@conference{wang13,
	Author = {Lingxiao Wang and Christian Boitet},
	Booktitle = {Workshop WPPT during MT Summit},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Online production of HQ parallel corpora and permanent task-based evaluation of multiple MT systems},
	Year = {2013}}

@inproceedings{Ueffing2003,
	Address = {New Orleans, LA},
	Author = {Nicola Ueffing and Klaus Macherey and Hermann Ney},
	Booktitle = {Proceedings of the MT Summit IX},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {September},
	Owner = {lent},
	Pages = {394-401},
	Timestamp = {2015.05.12},
	Title = {Confidence Measures for Statistical Machine Translation},
	Year = {2003}}

@inproceedings{ueffing07,
	Author = {Nicola Ueffing and Hermann Ney},
	Booktitle = {Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Number = {1},
	Pages = {9-40},
	Title = {Word-level confidence estimation for machine translation.},
	Volume = {33},
	Year = {2007}}

@inproceedings{ueffing05,
	Address = {Vancouver},
	Author = {Nicola Ueffing and Hermann Ney},
	Booktitle = {Proceedings of Human Language Technology Conference and Conference on Empirical Methods in Natural Language Processing},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {763--770},
	Title = {Word-level confidence estimation for machine translation using Phrased-based translation models},
	Year = {2005}}

@inproceedings{ueffing03,
	Address = {New Orleans, LA},
	Author = {Nicola Ueffing and Klaus Macherey and Hermann Ney},
	Booktitle = {Proceedings of the MT Summit IX},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {September},
	Pages = {394-401},
	Title = {Confidence Measures for Statistical Machine Translation},
	Year = {2003}}

@inproceedings{ueffing02,
	Address = {Philadelphia, PA},
	Author = {Nicola Ueffing and Franz Josef Och and Hermann Ney},
	Booktitle = {Proceedings of the Conference on Empirical Methods for Natural Language Processing (EMNLP 02)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {156-163},
	Title = {Generation of word graphs in statistical machine translation},
	Year = {2002}}

@conference{tromble2008,
	Author = {Roy Tromble and Shankar Kumar and Franz Josef Och and Wolfgang Macherey},
	Booktitle = {Lattice minimum bayesrisk Proceedings of the 2008 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {620-629},
	Title = {Lattice minimum bayes risk decoding for statistical machine translation.},
	Year = {2008}}

@conference{treetagger,
	Author = {Helmut Schmid},
	Booktitle = {International Conference on New Methods in Language Processing},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {44-49},
	Title = {Probabilistic Part-of-Speech Tagging Using Decision Trees},
	Year = {1994}}

@inproceedings{Stolcke2002,
	Address = {Denver, USA},
	Author = {Andreas Stolcke},
	Booktitle = {Seventh International Conference on Spoken Language Processing},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {lent},
	Pages = {901-904},
	Timestamp = {2015.05.12},
	Title = {SRILM - An Extensible Language Modeling Toolkit},
	Year = {2002}}

@inproceedings{stolcke02,
	Address = {Denver, USA},
	Author = {Andreas Stolcke},
	Booktitle = {Seventh International Conference on Spoken Language Processing},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {901-904},
	Title = {SRILM - An Extensible Language Modeling Toolkit},
	Year = {2002}}

@inproceedings{stolcke00,
	Author = {Stolcke, A and Klaus, R and Noah, C and Elizabeth, S and Rebecca, B and Daniel, J and Paul, T and Rachel, M and Marie, M and Carol, V},
	Booktitle = {Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {339-371},
	Title = {Dialogue Act Modeling for Automatic Tagging and Recognition of Conversational Speech},
	Year = {2000}}

@book{steven2009,
	Author = {Steven Bird and Ewan Klein and Edward Loper},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {lent},
	Publisher = {O'Reilly Media Inc},
	Timestamp = {2015.05.12},
	Title = {Natural Language Processing with Python},
	Year = {2009}}

@inproceedings{Specia2015,
	Author = {Specia, Lucia and Paetzold, G and Scarton, Carolina},
	Booktitle = {53rd Annual Meeting of the Association for Computational Linguistics and Seventh International Joint Conference on Natural Language Processing of the Asian Federation of Natural Language Processing: System Demonstrations},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {115--120},
	Title = {{Multi-level Translation Quality Prediction with QuEst++}},
	Year = {2015}}

@inproceedings{specia09b,
	Address = {Ottawa, Canada},
	Author = {Specia, L and Wang, Z and Turchi, M and Shawetaylor, J and Saunders, C},
	Booktitle = {Proceedings of the MT Summit XII},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Improving the confidence of machine translation quality estimates},
	Year = {2009}}

@inproceedings{specia09a,
	Address = {Barcelona},
	Author = {Specia, L and Turchi, M and Cancedda, N and Dymetman, M and Cristianini, N},
	Booktitle = {13th Conference of the European Association for Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {18-37},
	Title = {Estimating the Sentence-Level Quality of Machine Translation Systems},
	Year = {2009}}

@inproceedings{soricut10,
	Address = {Uppsala, Sweden},
	Author = {Radu Soricut and Abdessamad Echihabi},
	Booktitle = {Proceedings of the 48th annual meeting of the Association for Computational Linguistics)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {July},
	Pages = {612--621},
	Title = {Trustrank: Inducing trust in automatic translations via ranking},
	Year = {2010}}

@inproceedings{soricut02,
	Address = {London, UK},
	Author = {Radu Soricut and Kevin Knight and Daniel Marcu},
	Booktitle = {Proceedings of the 5th Conference of the Association for Machine Translation in the Americas on Machine Translation: From Research to Real Users},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Editor = {Springer-Verlag},
	Pages = {155-164},
	Title = {Using a large monolingual corpus to improve translation accuracy.},
	Year = {2002}}

@inproceedings{sokolov12b,
	Address = {Avignon, France},
	Author = {Artem Sokolov and Guillaume Wisniewski and Franc ?ois Yvon},
	Booktitle = {Proceedings of the 13th Conference of the European Chapter of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {April},
	Pages = {120-129},
	Title = {Computing Lattice BLEU Oracle Scores for Machine Translation},
	Year = {2012}}

@inproceedings{sokolov12,
	Author = {Artem Sokolov and Guillaume Wisniewski and Francois Yvon},
	Booktitle = {Proceedings of AMTA},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Non-linear n-best List Reranking with Few Features},
	Year = {2012}}

@inproceedings{Snover2008,
	Author = {Matthew Snover and Nitin Madnani and Bonnie Dorr and Richard Schwartz},
	Booktitle = {MetricsMATR workshop at AMTA},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {lent},
	Timestamp = {2015.05.12},
	Title = {TERp system description},
	Year = {2008}}

@inproceedings{snover08,
	Author = {Matthew Snover and Nitin Madnani and Bonnie Dorr and Richard Schwartz},
	Booktitle = {MetricsMATR workshop at AMTA},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {TERp system description},
	Year = {2008}}

@inproceedings{servan-toolkit-2015,
	Address = {Da Nang, Vietnam},
	Author = {Servan, Christophe and Le, Ngoc-Tien and Luong, Ngoc Quang and Lecouteux, Benjamin and Besacier, Laurent},
	Booktitle = {{The 12th International Workshop on Spoken Language Translation (IWSLT'15)}},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	File = {WCE_iwslt15.pdf:https\://hal.archives-ouvertes.fr/hal-01244477/file/WCE_iwslt15.pdf:PDF},
	Hal_Id = {hal-01244477},
	Hal_Version = {v1},
	Keywords = {Confidence Measures ; Quality Estimation ; SMT},
	Month = Dec,
	Title = {{An Open Source Toolkit for Word-level Confidence Estimation in Machine Translation}},
	Url = {https://hal.archives-ouvertes.fr/hal-01244477},
	Year = {2015},
	Bdsk-Url-1 = {https://hal.archives-ouvertes.fr/hal-01244477}}

@inproceedings{schmid1995,
	Address = {Dublin, Ireland},
	Author = {Helmut Schmid},
	Booktitle = {Proceedings of the ACL SIGDAT-Workshop},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {lent},
	Timestamp = {2015.05.11},
	Title = {Improvements in Part-of-Speech Tagging with an Application to German},
	Year = {1995}}

@inproceedings{sanchis07,
	Address = {Copenhagen, Denmark},
	Author = {Alberto Sanchis and Alfons Juan and Enrique Vidal},
	Booktitle = {Proceedings of the MT Summit XI},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {407-412},
	Title = {Estimation of confidence measures for machine translation},
	Year = {2007}}

@article{roberto2012,
	Author = {Roberto Navigli and Simone Paolo Ponzetto},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Artificial Intelligence},
	Owner = {Christophe},
	Pages = {217-250},
	Timestamp = {2015.06.05},
	Title = {BabelNet: The Automatic Construction, Evaluation and Application of a Wide-Coverage Multilingual Semantic Network},
	Volume = {193},
	Year = {2012}}

@article{raybaud2011,
	Author = {Sylvain Raybaud and David Langlois and Kamel Smaili},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Doi = {10.1007/s10590-011-9094-9},
	File = {cm-springer-utf8.pdf:https\://hal.archives-ouvertes.fr/hal-00606350/file/cm-springer-utf8.pdf:PDF},
	Hal_Id = {hal-00606350},
	Hal_Version = {v1},
	Journal = {Machine Translation},
	Keywords = {support vector machine ; mutual information ; partial least squares regression ; logistic regression ; neural network ; confidence measure ; translation evaluation ; machine translation},
	Month = Aug,
	Number = {1},
	Owner = {Christophe},
	Pages = {p. 1--34},
	Publisher = {{Springer Verlag (Germany)}},
	Timestamp = {2015.06.05},
	Title = {''This sentence is wrong.'' Detecting errors in machine-translated sentences},
	Volume = {25},
	Year = {2011},
	Bdsk-Url-1 = {https://hal.archives-ouvertes.fr/hal-00606350},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/s10590-011-9094-9}}

@inproceedings{raybaud09,
	Address = {Barcelona, Spain},
	Author = {Raybaud, S and Lavecchia, S and Langlois, D and Smaili, K},
	Booktitle = {Proceedings of the 13th EAMT},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {May},
	Title = {Error detection for statistical machine translation using linguistic features},
	Year = {2009}}


	
 

@inproceedings{Potet2012,
	Address = {Istanbul, Turkey},
	Author = {Potet, Marion and Esperan\c{c}a--Rodier , Emmanuelle and Besacier, Laurent and Blanchon, Herv\'e},
	Booktitle = {Proceedings of the eighth international conference on Language Resources and Evaluation (LREC)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {May},
	Owner = {lent},
	Timestamp = {2015.05.12},
	Title = {{Collection of a Large Database of French-English SMT Output Corrections}},
	Year = {2012}}

@inproceedings{Potet2010,
	Address = {Uppsala, Sweden},
	Author = {Potet, M and Besacier, L and Blanchon, H},
	Booktitle = {Proceedings of the joint fifth Workshop on Statistical Machine Translation and Metrics MATR (WMT2010)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Editor = {ACL Workshop},
	Month = {11-17 July},
	Owner = {lent},
	Timestamp = {2015.05.12},
	Title = {The LIG machine translation system for WMT 2010},
	Year = {2010}}

@inproceedings{potet12anonyme,
	Address = {Istanbul, Turkey},
	Author = {XX, Y.},
	Booktitle = {Proceedings of the eighth international conference on Language Resources and Evaluation (LREC)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {May},
	Title = {Collection of a Large Database of French-English SMT Output Corrections},
	Year = {2012}}

@inproceedings{potet12,
	Address = {Istanbul, Turkey},
	Author = {Potet, M and Emmanuelle E, R and Besacier, L and Blanchon, H},
	Booktitle = {Proceedings of the eighth international conference on Language Resources and Evaluation (LREC)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {May},
	Title = {Collection of a Large Database of French-English SMT Output Corrections},
	Year = {2012}}

@inproceedings{potet10anonyme,
	Address = {Uppsala, Sweden},
	Author = {XX, Y. and ZZ. W},
	Booktitle = {Proceedings of the joint fifth Workshop on Statistical Machine Translation and Metrics MATR (WMT2010)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Editor = {ACL Workshop},
	Month = {11-17 July},
	Title = {The XX machine translation system for WMT 2010},
	Year = {2010}}

@inproceedings{potet10,
	Address = {Uppsala, Sweden},
	Author = {Potet, M and Besacier, L and Blanchon, H},
	Booktitle = {Proceedings of the joint fifth Workshop on Statistical Machine Translation and Metrics MATR (WMT2010)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Editor = {ACL Workshop},
	Month = {11-17 July},
	Title = {The LIG machine translation system for WMT 2010},
	Year = {2010}}

@inproceedings{petrov2007,
	Author = {Slav Petrov and Dan Klein},
	Booktitle = {HLT-NAACL},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {lent},
	Timestamp = {2015.05.12},
	Title = {Improved Inference for Unlexicalized Parsing},
	Year = {2007}}

@inproceedings{papineni02,
	Author = {Kishore Papineni and Salim Roukos and Todd Ard and Wei-Jing Zhu},
	Booktitle = {Proceedings of the 40th Annual Meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {BLEU: a method for automatic evaluation of machine translation},
	Year = {2002}}

@article{och2003,
	Author = {Franz Josef Och and Hermann Ney},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Computational Linguistics},
	Number = {1},
	Owner = {Christophe},
	Pages = {19--51},
	Timestamp = {2015.06.05},
	Title = {A Systematic Comparison Of Various Statistical Alignment Models},
	Volume = {29},
	Year = {2003}}

@inproceedings{och03,
	Author = {Franz Josef Och},
	Booktitle = {Proceedings of the 41st Annual Meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {July},
	Pages = {160-167},
	Title = {Minimum Error Rate Training in Statistical Machine Translation},
	Year = {2003}}

@inproceedings{nguyen11,
	Address = {Portland, Oregon},
	Author = {Bach Nguyen and Fei Huang and Yaser Al-Onaizan},
	Booktitle = {Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Pages = {211--219},
	Title = {Goodness: A Method for Measuring Machine Translation Confidence},
	Year = {2011}}

@inproceedings{ngocquang:hal-01002922anonyme,
	Address = {Dubrovnik, Croatie},
	Author = {XX, Y},
	Booktitle = {{E}uropean {A}ssociation for {M}achine {T}ranslation ({EAMT})},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {jun},
	Title = {{A}n {E}fficient {T}wo-{P}ass {D}ecoder for {SMT} {U}sing {W}ord {C}onfidence {E}stimation},
	Url = {http://hal.inria.fr/hal-01002922},
	X-International-Audience = {yes},
	Year = {2014},
	Bdsk-Url-1 = {http://hal.inria.fr/hal-01002922}}

@inproceedings{ngocquang:hal-01002922,
	Address = {Dubrovnik, Croatie},
	Author = {Luong, Ngoc Quang and Besacier, Laurent and Lecouteux, Benjamin},
	Booktitle = {{E}uropean {A}ssociation for {M}achine {T}ranslation ({EAMT})},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {jun},
	Title = {{A}n {E}fficient {T}wo-{P}ass {D}ecoder for {SMT} {U}sing {W}ord {C}onfidence {E}stimation},
	Url = {http://hal.inria.fr/hal-01002922},
	X-International-Audience = {yes},
	Year = {2014},
	Bdsk-Url-1 = {http://hal.inria.fr/hal-01002922}}

@inproceedings{nakov12,
	Address = {Mumbai, India},
	Author = {Preslav Nakov and Francisco Guzman and Stephan Vogel},
	Booktitle = {Proceedings of COLING 2012},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {December 8 -15},
	Pages = {1979-1994},
	Title = {Optimizing for Sentence-Level BLEU+1 Yields Short Translations},
	Year = {2012}}

@conference{mikolov2013,
	Author = {Tomas Mikolov and Ilya Sutskever and Kai Chen and Greg Corrado and Jeffrey Dean},
	Booktitle = {NIPS},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {Christophe},
	Timestamp = {2015.09.24},
	Title = {Distributed Representations of Words and Phrases and their Compositionality},
	Year = {2013}}

@article{luong15,
	Author = {Ngoc-Quang Luong and Laurent Besacier and Benjamin Lecouteux},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Data and Knowledge Engineering},
	Keywords = {quality estimation ; word confidence estimation ; ; statistical machine translation},
	Month = Apr,
	Pages = {11},
	Publisher = {{Elsevier}},
	Title = {Towards Accurate Predictors of Word Quality for Machine Translation: Lessons Learned on French - English and English - Spanish Systems},
	Year = {2015}}

@inproceedings{luong14,
	Address = {Gothenburg, Sweden},
	Author = {Ngoc Quang Luong and Laurent Besacier and Benjamin Lecouteux},
	Booktitle = {Proceedings of the Workshop on Humans and Computer-assisted Translation (HaCaT)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {April},
	Title = {Word Confidence Estimation for SMT N-best List Re-ranking},
	Year = {2014}}

@inproceedings{luong13b,
	Address = {Sofia, Bulgaria},
	Author = {Luong, Ngoc Quang and Lecouteux, Benjamin and Besacier, Laurent},
	Booktitle = {Proceedings of the Eighth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {August},
	Pages = {396--391},
	Publisher = {Association for Computational Linguistics},
	Title = {{LIG} System for {WMT}13 {QE} Task: Investigating the Usefulness of Features in Word Confidence Estimation for {MT}},
	Year = {2013}}

@inproceedings{luong13anonyme,
	Address = {Hanoi, Vietnam},
	Author = {XX, Y.},
	Booktitle = {Proceedings of The Fifth International Conference on Knowledge and Systems Engineering (KSE 2013)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {October 17-19},
	Title = {Word Confidence Estimation and its Integration in Sentence Quality Estimation for Machine Translation},
	Year = {2013}}

@inproceedings{luong13,
	Address = {Hanoi, Vietnam},
	Author = {Ngoc Quang Luong and Laurent Besacier and Benjamin Lecouteux},
	Booktitle = {Proceedings of The Fifth International Conference on Knowledge and Systems Engineering (KSE 2013)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {October 17-19},
	Title = {Word Confidence Estimation and its Integration in Sentence Quality Estimation for Machine Translation},
	Year = {2013}}

@inproceedings{luong:hal-00953719,
	Abstract = {no abstract},
	Address = {Gothenburg, Su{\`e}de},
	Author = {Luong, Ngoc-Quang and Besacier, Laurent and Lecouteux, Benjamin},
	Booktitle = {{P}roceedings of the {W}orkshop on {H}umans and {C}omputer-assisted {T}ranslation ({H}a{C}a{T}) during {EACL}},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {{W}ord {C}onfidence {E}stimation for {SMT} {N}-best {L}ist {R}e-ranking},
	Url = {http://hal.inria.fr/hal-00953719},
	X-International-Audience = {yes},
	Year = {2014},
	Bdsk-Url-1 = {http://hal.inria.fr/hal-00953719}}

@inproceedings{luong_wmt14,
	Address = {Baltimore, Maryland USA},
	Author = {Ngoc-Quang Luong and Laurent Besacier and Benjamin Lecouteux},
	Booktitle = {Proceedings of the Ninth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = jun,
	Owner = {lent},
	Pages = {335--341},
	Timestamp = {2015.06.04},
	Title = {{LIG System for Word Level QE task at WMT14}},
	Year = {2014}}

@article{Lecouteux2011,
	Author = {Benjamin Lecouteux and Georges Linares and Stanislas Oger},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Computer Speech and Language},
	Title = {Integrating imperfect transcripts into speech recognition systems for building high-quality corpora},
	Year = {2011}}

@article{Lecouteux2009,
	Author = {Lecouteux, Benjamin and Linar{\`e}s, Georges and Favre, Benoit},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {INTERSPEECH},
	Title = {Combined low level and high level features for Out-Of-Vocabulary Word detection},
	Year = {2009}}

@inproceedings{Lavergne2010,
	Author = {Lavergne, Thomas and Capp\'{e}, Olivier and Yvon, Fran\c{c}ois},
	Booktitle = {Proceedings the 48th Annual Meeting of the Association for Computational Linguistics ({ACL})},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Location = {Uppsala, Sweden},
	Month = {July},
	Pages = {504--513},
	Publisher = {Association for Computational Linguistics},
	Title = {Practical Very Large Scale {CRFs}},
	Year = {2010}}

@inproceedings{lavergne10,
	Author = {Thomas Lavergne and Olivier Capp\'e and Fran\c{c}ois Yvon},
	Booktitle = {Proceedings of the 48th Annual Meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {504-513},
	Title = {Practical very large scale CRFs},
	Year = {2010}}

@inproceedings{Laurent2014a,
	Address = {Singapour},
	Author = {Antoine Laurent and Nathalie Camelin and Christian Raymond},
	Booktitle = {InterSpeech},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {September},
	Owner = {Christophe},
	Pages = {76-80},
	Timestamp = {2015.09.24},
	Title = {Boosting bonsai trees for efficient features combination: application to speaker role identification},
	Year = {2014}}

@inproceedings{langlois12,
	Address = {Baltimore, Maryland USA},
	Author = {David Langlois and Sylvain Raybaud and Kamel Sma{\"\i}li},
	Booktitle = {Proceedings of the Seventh Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = jun,
	Owner = {Christophe},
	Pages = {114--119},
	Timestamp = {2015.09.24},
	Title = {Loria system for the WMT12 quality estimation shared task},
	Year = {2012}}

@article{lamel1991bref,
	Author = {Lamel, Lori F and Gauvain, Jean-Luc and Esk{\'e}nazi, Mazcine and others},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {training},
	Number = {28},
	Pages = {50},
	Title = {BREF, a Large Vocabulary Spoken Corpus for French1},
	Volume = {22},
	Year = {1991}}

@inproceedings{Lafferty2001,
	Author = {John Lafferty and Andrew McCallum and Fernando Pereira},
	Biburl = {http://www.bibsonomy.org/bibtex/2093b1a44f0715eb0183df4606a0feaff/arath},
	Booktitle = {{P}roceedings of 18th International Conference on Machine Learning},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Keywords = {kernel},
	Owner = {Christophe},
	Pages = {282--289},
	Publisher = {Morgan Kaufmann, San Francisco, Californie, \'Etats-Unis d'Am{\'e}rique},
	Timestamp = {2015.09.24},
	Title = {Conditional Random Fields: {P}robabilistic Models for Segmenting and Labeling Sequence Data},
	Year = {2001}}

@inproceedings{lafferty01,
	Author = {John Lafferty and Andrew McCallum and Fernando Pereira},
	Booktitle = {Proceedings of ICML-01},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {282-289},
	Title = {Conditional random fields: Probabilistic models for segmenting et labeling sequence data},
	Year = {2001}}

@article{Kudo2000a,
	Author = {Kudo, Mineichi and Sklansky, Jack},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Pattern recognition},
	Number = {1},
	Owner = {Christophe},
	Pages = {25--41},
	Publisher = {Elsevier},
	Timestamp = {2015.09.14},
	Title = {Comparison of algorithms that select features for pattern classifiers},
	Volume = {33},
	Year = {2000}}

@article{Kudo2000,
	Author = {Kudo, Mineichi and Sklansky, Jack},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Pattern recognition},
	Number = {1},
	Owner = {Christophe},
	Pages = {25--41},
	Publisher = {Elsevier},
	Timestamp = {2015.09.14},
	Title = {Comparison of algorithms that select features for pattern classifiers},
	Volume = {33},
	Year = {2000}}

@inproceedings{kristen12,
	Address = {Trento, Italy},
	Author = {Kristen Parton and Nizar Habash and Kathleen McKeown and Gonzalo Iglesias and Adri{\`a} de Gispert},
	Booktitle = {Proceedings of the 16th EAMT},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {28-30 May},
	Pages = {111-118},
	Title = {Can Automatic Post-Editing Make MT More Meaningful?},
	Year = {2012}}

@inproceedings{Koehn2007,
	Address = {Prague, Czech Republic},
	Author = {Philipp Koehn and Hieu Hoang and Alexandra Birch and Chris Callison-Burch and Marcello Federico and Nicola Bertoldi and Brooke Cowan and Wade Shen and Christine Moran and Richard Zens and Chris Dyer and Ondrej Bojar and Alexandra Constantin and Evan Herbst},
	Booktitle = {Proceedings of the 45th Annual Meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Owner = {lent},
	Pages = {177-180},
	Rating = {5},
	Read = {1},
	Timestamp = {2015.05.12},
	Title = {Moses: Open source toolkit for statistical machine translation},
	Year = {2007}}

@inproceedings{koehn07,
	Address = {Prague, Czech Republic},
	Author = {Philipp Koehn and Hieu Hoang and Alexandra Birch and Chris Callison-Burch and Marcello Federico and Nicola Bertoldi and Brooke Cowan and Wade Shen and Christine Moran and Richard Zens and Chris Dyer and Ondrej Bojar and Alexandra Constantin and Evan Herbst},
	Booktitle = {Proceedings of the 45th Annual Meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Pages = {177-180},
	Rating = {5},
	Read = {1},
	Title = {Moses: Open source toolkit for statistical machine translation},
	Year = {2007}}

@inproceedings{kirchhoff05,
	Address = {Ann Arbor, Michigan},
	Author = {Katrin Kirchhoff and Mei Yang},
	Booktitle = {Proceedings of the ACL Workshop on Building and Using Parallel Texts},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Pages = {125-128},
	Title = {Improved Language Modeling for Statistical Machine Translation},
	Year = {2005}}

@article{Kemp1997,
	Author = {Kemp, Thomas and Schaaf, Thomas},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Proc. of European Conference on Speech Communication Technology},
	Pages = {827-830},
	Title = {ESTIMATING CONFIDENCE USING WORD LATTICES},
	Year = {1997}}

@inproceedings{JulienFayolle2010,
	Author = {Julien Fayolle and Fabienne Moreau and Christian Raymond and Guillaume Gravier and Patrick Gros},
	Booktitle = {Interspeech},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {assyrium},
	Timestamp = {2014.09.24},
	Title = {CRF-based combination of contextual features to improve a posteriori word-level confidence measures.},
	Year = {2010}}

@article{Jiang2004,
	Author = {Jiang, Hui},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Speech Communication},
	Title = {Confidence measures for speech recognition: A survey},
	Year = {2004}}

 
@inproceedings{iwslt2012_campaign,
	Author = {Federico, Marcello and Cettolo, Mauro and Bentivogli, Luisa and Paul, Michael and St\"{u}ker, Sebastian},
	Booktitle = {{I}n proceedings of the 9th {I}nternational {W}orkshop on {S}poken {L}anguage {T}ranslation ({IWSLT})},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {December},
	Title = {Overview of the {IWSLT} 2012 Evaluation Campaign},
	Year = {2012}}

@inproceedings{hildebrand05,
	Address = {Budapest},
	Author = {Almut Silja Hildebrand and Matthias Eck and Stephan Vogel and Alex Waibel},
	Booktitle = {Proceedings of the 10th EAMT conference ''Practical applications of machine translation''},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {May},
	Pages = {133-142},
	Title = {Adaptation of the Translation Model for Statistical Machine Translation based on Information Retrieval},
	Year = {2005}}

@inproceedings{Han2013,
	Address = {Sofia, Bulgaria},
	Author = {Han, Aaron Li-Feng and Lu, Yi and Wong, Derek F and Chao, Lidia S and He, Liangye and Xing, Junwen},
	Booktitle = {Proceedings of the Eighth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = aug,
	Owner = {Christophe},
	Pages = {365--372},
	Timestamp = {2015.09.24},
	Title = {Quality estimation for machine translation using the joint method of evaluation criteria and statistical modeling},
	Year = {2013}}

@inproceedings{han13,
	Address = {Sofia, Bulgaria},
	Author = {Han, Aaron Li-Feng and Lu, Yi and Wong, Derek F. and Chao, Lidia S. and He, Liangye and Xing, Junwen},
	Booktitle = {Proceedings of the Eighth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {August},
	Pages = {365--372},
	Publisher = {Association for Computational Linguistics},
	Title = {Quality Estimation for Machine Translation Using the Joint Method of Evaluation Criteria and Statistical Modeling},
	Url = {http://www.aclweb.org/anthology/W13-2245},
	Year = {2013},
	Bdsk-Url-1 = {http://www.aclweb.org/anthology/W13-2245}}

@inproceedings{gandrabur03,
	Address = {Edmonton},
	Author = {Simona Gandrabur and George Foster},
	Booktitle = {Proceedings of the Conference on Natural Language Learning (CoNLL 2003)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {May},
	Pages = {315-321},
	Title = {Confidence estimation for text prediction},
	Year = {2003}}

@inproceedings{Galliano06corpusdescription,
	Author = {Sylvain Galliano and Edouard Geoffrois and Guillaume Gravier and Jean-Francois Bonastre and Djamel Mostefa and Khalid Choukri},
	Booktitle = {In Proceedings of the 5th international Conference on Language Resources and Evaluation (LREC 2006)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Pages = {315--320},
	Title = {Corpus description of the ester evaluation campaign for the rich transcription of french broadcast news},
	Year = {2006}}

@phdthesis{frank04,
	Address = {Belgium},
	Author = {Frank Vanden Berghen},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	School = {University of Brussels (ULB - Universit{\'e} Libre de Bruxelles)},
	Title = {CONDOR: a constrained, non-linear, derivative-free parallel optimizer for continuous, high computing load, noisy objective functions},
	Year = {2004}}

@inproceedings{Felice2012,
	Address = {Montreal, Canada},
	Author = {Mariano Felice and Lucia Specia},
	Booktitle = {Proceedings of the 7th Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June 7-8},
	Owner = {lent},
	Pages = {96-103},
	Timestamp = {2015.05.12},
	Title = {Linguistic Features for Quality Estimation},
	Year = {2012}}

@inproceedings{felice12,
	Address = {Montreal, Canada},
	Author = {Mariano Felice and Lucia Specia},
	Booktitle = {Proceedings of the 7th Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June 7-8},
	Pages = {96-103},
	Title = {Linguistic Features for Quality Estimation},
	Year = {2012}}

@inproceedings{eamt2014,
	Address = {Dubrovnik, Croatie},
	Author = {Luong, Ngoc Quang and Besacier, Laurent and Lecouteux, Benjamin},
	Booktitle = {{E}uropean {A}ssociation for {M}achine {T}ranslation ({EAMT})},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {jun},
	Title = {{A}n {E}fficient {T}wo-{P}ass {D}ecoder for {SMT} {U}sing {W}ord {C}onfidence {E}stimation},
	Url = {http://hal.inria.fr/hal-01002922},
	X-International-Audience = {yes},
	Year = {2014},
	Bdsk-Url-1 = {http://hal.inria.fr/hal-01002922}}

@inproceedings{Duh08,
	Author = {Kevin Duh and Katrin Kirchhoff},
	Booktitle = {Proc. of ACL, Short Papers},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Beyond Log-Linear Models: Boosted Minimum Error Rate Training for N-best Re-ranking},
	Year = {2008}}

@conference{decodeEMNLP2013,
	Author = {Ashish Vaswani and Yinggong Zhao and Victoria Fossum and David Chiang},
	Booktitle = {Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Decoding with Large-Scale Neural Language Models Improves Translation},
	Year = {2013}}

@inproceedings{collins05,
	Address = {Ann Arbor},
	Author = {Michael Collins and Philipp Koehn and Ivona Kuc?erova ?},
	Booktitle = {Proceedings of the 43rd Annual Meeting of the ACL},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Pages = {531-540},
	Title = {Clause Restructuring for Statistical Machine Translation},
	Year = {2005}}

@conference{Clark2011,
	Address = {Portland, Oregon},
	Author = {Clark, Jonathan H. and Dyer, Chris and Lavie, Alon and Smith, Noah A.},
	Booktitle = {Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics: Human Language Technologies: Short Papers - Volume 2},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Editor = {Association for Computational Linguistics},
	Pages = {176--181},
	Title = {Better Hypothesis Testing for Statistical Machine Translation: Controlling for Optimizer Instability},
	Year = {2011}}

@inproceedings{clark11,
	Author = {Jonathan Clark and Chris Dyer and Alon Lavie and Noah Smith},
	Booktitle = {Proceedings of the Association for Computational Lingustics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Better Hypothesis Testing for Statistical Machine Translation: Controlling for Optimizer Instability},
	Year = {2011}}

@conference{Parton:fk,
	Author = {Parton, K},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000}}

@inproceedings{CCB2012,
	Address = {Montr{\'e}al, Canada},
	Author = {Callison-Burch, Chris and Koehn, Philipp and Monz, Christof and Post, Matt and Soricut, Radu and Specia, Lucia},
	Booktitle = {Proceedings of the Seventh Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Owner = {Christophe},
	Pages = {10--51},
	Publisher = {Association for Computational Linguistics},
	Timestamp = {2015.09.24},
	Title = {Findings of the 2012 Workshop on Statistical Machine Translation},
	Year = {2012}}

@manual{capit13,
	Address = {Laboratoire d'Informatique de Grenoble Bat. ENSIMAG - antenne de Montbonnot ZIRST 51, avenue Jean Kuntzmann 38330 MONTBONNOT SAINT MARTIN},
	Author = {Capit Nicolas and Emeras Joseph},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Organization = {LIG laboratory},
	Title = {OAR Documentation - User Guide},
	Year = {2013}}

@inproceedings{candito2010,
	Author = {Marie Candito and Joakim Nivre and Pascal Denis and Enrique Henestroza Anguiano},
	Booktitle = {Proceedings of COLING'2010},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {lent},
	Timestamp = {2015.06.04},
	Title = {Benchmarking of Statistical Dependency Parsers for French},
	Year = {2010}}

@inproceedings{CamargodeSouza2014,
	Address = {Baltimore, Maryland, USA},
	Author = {Camargo de Souza, Jos\'{e} Guilherme and Gonz\'{a}lez-Rubio, Jes\'{u}s and Buck, Christian and Turchi, Marco and Negri, Matteo},
	Booktitle = {Proceedings of the Ninth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Owner = {Christophe},
	Pages = {322--328},
	Publisher = {Association for Computational Linguistics},
	Timestamp = {2015.09.24},
	Title = {FBK-UPV-UEdin participation in the WMT14 Quality Estimation shared-task},
	Year = {2014}}

@proceedings{brown93a,
	Author = {Brown, PF and Stephen, A and Pietra, V and Robert, LM},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Editor = {Computational Linguistics},
	Number = {263-311},
	Title = {The mathematics of statistical machine translation: parameter estimation},
	Volume = {19},
	Year = {1993a}}

@proceedings{brown93a,
	Author = {Brown, PF and Stephen, A and Pietra, V and Robert, LM},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Editor = {Computational Linguistics},
	Number = {263-311},
	Title = {The mathematics of statistical machine translation: parameter estimation},
	Volume = {19},
	Year = {1993a}}

@inproceedings{Bojar2014,
	Address = {Baltimore, Maryland, USA},
	Author = {Bojar, Ondrej and Buck, Christian and Federmann, Christian and Haddow, Barry and Koehn, Philipp and Leveling, Johannes and Monz, Christof and Pecina, Pavel and Post, Matt and Saint-Amand, Herve and Soricut, Radu and Specia, Lucia and Tamchyna, Ale\v{s}},
	Booktitle = {Proceedings of the Ninth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Owner = {Christophe},
	Pages = {12--58},
	Publisher = {Association for Computational Linguistics},
	Timestamp = {2015.09.24},
	Title = {Findings of the 2014 Workshop on Statistical Machine Translation},
	Year = {2014}}

@inproceedings{bojar2013,
	Address = {Sofia, Bulgaria},
	Author = {Bojar, Ond\v{r}ej and Buck, Christian and Callison-Burch, Chris and Federmann, Christian and Haddow, Barry and Koehn, Philipp and Monz, Christof and Post, Matt and Soricut, Radu and Specia, Lucia},
	Booktitle = {Proceedings of the Eighth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {August},
	Owner = {lent},
	Pages = {1--44},
	Publisher = {Association for Computational Linguistics},
	Timestamp = {2015.05.12},
	Title = {Findings of the 2013 {Workshop on Statistical Machine Translation}},
	Year = {2013},
	Bdsk-Url-1 = {http://www.aclweb.org/anthology/W13-2201}}

@inproceedings{blatz2004,
	Address = {Geneva},
	Author = {John Blatz and Erin Fitzgerald and George Foster and Simona Gandrabur and Cyril Goutte and Alex Kulesza and Alberto Sanchis and Nicola Ueffing},
	Booktitle = {Proceedings of COLING 2004},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Institution = {The JHU Workshop Final Report},
	Month = {April},
	Pages = {315-321},
	Title = {Confidence estimation for machine translation},
	Year = {2004}}

@techreport{blatz2003,
	Author = {John Blatz and Erin Fitzgerald and George Foster and Simona Gandrabur and Cyril Goutte and Alex Kulesza and Alberto Sanchis and Nicola Ueffing},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Institution = {JHU/CLSP Summer Workshop},
	Title = {Confidence estimation for machine translation},
	Year = {2003}}

@inproceedings{blatz04,
	Address = {Geneva},
	Author = {John Blatz and Erin Fitzgerald and George Foster and Simona Gandrabur and Cyril Goutte and Alex Kulesza and Alberto Sanchis and Nicola Ueffing},
	Booktitle = {Proceedings of COLING 2004},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Institution = {The JHU Workshop Final Report},
	Month = {April},
	Owner = {lent},
	Pages = {315-321},
	Timestamp = {2015.05.12},
	Title = {Confidence estimation for machine translation},
	Year = {2004}}

@inproceedings{Bicici2013,
	Address = {Sofia, Bulgaria},
	Author = {Bicici, Ergun},
	Booktitle = {Proceedings of the Eighth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {August},
	Pages = {343--351},
	Publisher = {Association for Computational Linguistics},
	Title = {Referential Translation Machines for Quality Estimation},
	Year = {2013}}

@inproceedings{bicici13,
	Address = {Sofia, Bulgaria},
	Author = {Bicici, Ergun},
	Booktitle = {Proceedings of the Eighth Workshop on Statistical Machine Translation},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {August},
	Pages = {343--351},
	Publisher = {Association for Computational Linguistics},
	Title = {Referential Translation Machines for Quality Estimation},
	Url = {http://www.aclweb.org/anthology/W13-2242},
	Year = {2013},
	Bdsk-Url-1 = {http://www.aclweb.org/anthology/W13-2242}}

@inproceedings{besacier14anonyme,
	Address = {Lake Tahoe, USA},
	Author = {X Y and W Z},
	Booktitle = {Proceedings of The International Workshop on Spoken Language Translation (IWSLT)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {December},
	Title = {Word Confidence Estimation for Speech Translation},
	Year = {2014}}

@inproceedings{besacier14,
	Address = {Lake Tahoe, USA},
	Author = {Laurent Besacier and Benjamin Lecouteux and Ngoc Quang Luong and Kaing Hour and Marwa Hadjsalah},
	Booktitle = {Proceedings of The International Workshop on Spoken Language Translation (IWSLT)},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {December},
	Title = {Word Confidence Estimation for Speech Translation},
	Year = {2014}}

@inproceedings{besacier-asru-2015,
	Address = {Scotsdale, Arizona, United States},
	Author = {Besacier, Laurent and Lecouteux, Benjamin and Luong, Ngoc-Quang and Le, Ngoc-Tien},
	Booktitle = {{IEEE Workshop on Automatic Speech Recognition and Understanding (ASRU)}},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Doi = {10.1109/ASRU.2015.7404804},
	Hal_Id = {hal-01289158},
	Hal_Version = {v1},
	Keywords = {Quality estimation ; Search graph re-decoding ; Spoken Language Translation (SLT) ; Word confidence estimation (WCE)},
	Month = Dec,
	Title = {{Spoken language translation graphs re-decoding using automatic quality assessment}},
	Url = {https://hal.archives-ouvertes.fr/hal-01289158},
	Year = {2015},
	Bdsk-Url-1 = {https://hal.archives-ouvertes.fr/hal-01289158},
	Bdsk-Url-2 = {http://dx.doi.org/10.1109/ASRU.2015.7404804}}

@inproceedings{Bach2011,
	Address = {Portland, Oregon},
	Author = {Bach, Nguyen and Huang, Fei and Al-Onaizan, Yaser},
	Booktitle = {Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June},
	Owner = {lent},
	Pages = {211--219},
	Timestamp = {2015.05.12},
	Title = {Goodness: A Method for Measuring Machine Translation Confidence},
	Year = {2011}}

@inproceedings{bach11,
	Address = {Portland, Oregon},
	Author = {Nguyen Bach and Fei Huang and Yaser Al-Onaizan},
	Booktitle = {Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {June 19-24},
	Pages = {211-219},
	Title = {Goodness: A Method for Measuring Machine Translation Confidence},
	Year = {2011}}

@inproceedings{ashish07,
	Author = {Ashish Venugopal and Andreas Zollmann and Stephan Vogel},
	Booktitle = {Proceedings of Human Language Technologies 2007: The Conference of the North American Chapter of the Association for Computational Linguistics},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Month = {April},
	Title = {An Efficient Two-Pass Approach to Synchronous-CFG Driven Statistical MT},
	Year = {2007}}

@article{Asadi1990,
	Author = {Ayman Asadi and Richard Schwartz and John Makhoul},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Journal = {Proc. of International Conference on Acoustics, Speech and Signal Processing},
	Title = {Automatic detection of new words in a large vocabulary continuous speech recognition system},
	Year = {1990}}

@inproceedings{AntoineLaurent2014,
	Author = {Antoine Laurent and Nathalie Camelin and Christian Raymond},
	Booktitle = {Interspeech},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Owner = {assyrium},
	Timestamp = {2014.09.24},
	Title = {Boosting bonsai trees for efficient features combination : application to speaker role identification},
	Year = {2014}}

@inproceedings{anonymZ,
	Author = {Anonym\_Z and Anonym\_Z1 and Anonym\_Z2},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Anonymous Title},
	Year = {2013}}

@inproceedings{anonymY,
	Author = {Anonym\_Y and Anonym\_Y1 and Anonym\_Y2},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Anonymous Title},
	Year = {2012}}

@inproceedings{anonymX,
	Author = {Anonym\_X and Anonym\_X1 and Anonym\_X2},
	Date-Added = {2017-03-17 16:15:25 +0000},
	Date-Modified = {2017-03-17 16:15:25 +0000},
	Title = {Anonymous Title},
	Year = {2013}}

@inproceedings{povey2011kaldi,
	Author = {Povey, Daniel and Ghoshal, Arnab and Boulianne, Gilles and Burget, Lukas and Glembek, Ondrej and Goel, Nagendra and Hannemann, Mirko and Motlicek, Petr and Qian, Yanmin and Schwarz, Petr and others},
	Booktitle = {IEEE 2011 workshop on automatic speech recognition and understanding},
	Number = {EPFL-CONF-192584},
	Organization = {IEEE Signal Processing Society},
	Title = {The Kaldi speech recognition toolkit},
	Year = {2011}}

@article{jalalvand2016transcrater,
	Author = {Jalalvand, Shahab and Negri, Matteo and Turchi, Marco and de Souza, Jos{\'e} GC and Falavigna, Daniele and Qwaider, Mohammed RH},
	Journal = {Proceedings of ACL-2016 System Demonstrations. Berlin, Germany: Association for Computational Linguistics},
	Pages = {43--48},
	Title = {Transcrater: a tool for automatic speech recognition quality estimation},
	Year = {2016}}
 

@inproceedings{stolcke2002srilm,
	Author = {Stolcke, Andreas and others},
	Booktitle = {Interspeech},
	Pages = {2002},
	Title = {SRILM-an extensible language modeling toolkit.},
	Volume = {2002},
	Year = {2002}}

@inproceedings{galliano2005ester,
	Author = {Galliano, Sylvain and Geoffrois, Edouard and Mostefa, Djamel and Choukri, Khalid and Bonastre, Jean-Fran{\c{c}}ois and Gravier, Guillaume},
	Booktitle = {Interspeech},
	Pages = {1149--1152},
	Title = {The ESTER phase II evaluation campaign for the rich transcription of French broadcast news.},
	Year = {2005}}

@inproceedings{kahn2012presentation,
	Author = {Kahn, Juliette and Galibert, Olivier and Quintard, Ludovic and Carr{\'e}, Matthieu and Giraudel, Aude and Joly, Philippe},
	Booktitle = {Content-Based Multimedia Indexing (CBMI), 2012 10th International Workshop on},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A presentation of the REPERE challenge},
	Year = {2012}}

@inproceedings{gravier2012etape,
	Author = {Gravier, Guillaume and Adda, Gilles and Paulson, Niklas and Carr{\'e}, Matthieu and Giraudel, Aude and Galibert, Olivier},
	Booktitle = {LREC-Eighth international conference on Language Resources and Evaluation},
	Pages = {na},
	Title = {The ETAPE corpus for the evaluation of speech-based TV content processing in the French language},
	Year = {2012}}

@article{hinton2012improving,
	Author = {Hinton, Geoffrey E and Srivastava, Nitish and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan R},
	Journal = {arXiv preprint arXiv:1207.0580},
	Title = {Improving neural networks by preventing co-adaptation of feature detectors},
	Year = {2012}}

@inproceedings{negri2014quality,
	Author = {Negri, Matteo and Turchi, Marco and de Souza, Jos{\'e} GC and Falavigna, Daniele},
	Booktitle = {COLING},
	Pages = {1813--1823},
	Title = {Quality Estimation for Automatic Speech Recognition.},
	Year = {2014}}

@inproceedings{de1998bdlex,
	Author = {De Calm{\`e}s, Martine and P{\'e}rennou, Guy},
	Booktitle = {Proceedings of 1st International Conference on Langage Resources \& Evaluation},
	Pages = {1129--1136},
	Title = {BDLEX: a lexicon for spoken and written French},
	Year = {1998}}

@article{schmid1995treetagger,
	Author = {Schmid, Helmut},
	Journal = {Institut f{\"u}r Maschinelle Sprachverarbeitung, Universit{\"a}t Stuttgart},
	Pages = {28},
	Title = {Treetagger| a language independent part-of-speech tagger},
	Volume = {43},
	Year = {1995}
	}
	

@inproceedings{specia2013quest,
  title={QuEst-A translation quality estimation framework.},
  author={Specia, Lucia and Shah, Kashif and De Souza, Jos{\'e} GC and Cohn, Trevor},
  booktitle={ACL (Conference System Demonstrations)},
  pages={79--84},
  year={2013},
  organization={Citeseer}
}

@inproceedings{conf/interspeech/Galibert13a,
  added-at = {2014-01-27T00:00:00.000+0100},
  author = {Galibert, Olivier},
  biburl = {http://www.bibsonomy.org/bibtex/27e9c4b156bead221594002fdb1885c71/dblp},
  booktitle = {INTERSPEECH},
  editor = {Bimbot, Fr�d�ric and Cerisara, Christophe and Fougeron, C�cile and Gravier, Guillaume and Lamel, Lori and Pellegrino, Fran�ois and Perrier, Pascal},
  ee = {http://www.isca-speech.org/archive/interspeech_2013/i13_1131.html},
  interhash = {9e7a9230a2f78ed7025e2876940fa20c},
  intrahash = {7e9c4b156bead221594002fdb1885c71},
  keywords = {dblp},
  pages = {1131-1134},
  publisher = {ISCA},
  timestamp = {2014-01-28T11:37:31.000+0100},
  title = {Methodologies for the evaluation of speaker diarization and automatic speech recognition in the presence of overlapping speech.},
  url = {http://dblp.uni-trier.de/db/conf/interspeech/interspeech2013.html#Galibert13a},
  year = 2013
}
@misc{chollet2015keras,
	  title={Keras},
	    author={Chollet, Fran\c{c}ois and others},
	      year={2015},
	        publisher={GitHub},
		  howpublished={\url{https://github.com/fchollet/keras}},
}
@misc{tensorflow2015-whitepaper,
	title={ {TensorFlow}: Large-Scale Machine Learning on Heterogeneous Systems},
	url={https://www.tensorflow.org/},
	note={Software available from tensorflow.org},
	author={
		    Mart\'{\i}n~Abadi and
			        Ashish~Agarwal and
				    Paul~Barham and Xiaoqiang~Zheng et al},
	  year={2015},
}
@inproceedings{mcfee2015librosa,
	  title={librosa: Audio and music signal analysis in python},
	    author={McFee, Brian and Raffel, Colin and Liang, Dawen and Ellis, Daniel PW and McVicar, Matt and Battenberg, Eric and Nieto, Oriol},
	      year={2015}
}
@inproceedings{Eyben:2010:OMV:1873951.1874246,
	 author = {Eyben, Florian and W\"{o}llmer, Martin and Schuller, Bj\"{o}rn},
	  title = {Opensmile: The Munich Versatile and Fast Open-source Audio Feature Extractor},
	   booktitle = {Proceedings of the 18th ACM International Conference on Multimedia},
	    series = {MM '10},
	     year = {2010},
	      isbn = {978-1-60558-933-6},
	       location = {Firenze, Italy},
	        pages = {1459--1462},
		 numpages = {4},
		  url = {http://doi.acm.org/10.1145/1873951.1874246},
		   doi = {10.1145/1873951.1874246},
		    acmid = {1874246},
		     publisher = {ACM},
		      address = {New York, NY, USA},
		       keywords = {audio feature extraction, emotion, music, signal processing, speech, statistical functionals},
} 


